Unlearning during Learning: An Efficient Federated Machine Unlearning Method

In recent years, Federated Learning (FL) has garnered significant attention as a distributed machine learning paradigm. To facilitate the implementation of the right to be forgotten, the concept of federated machine unlearning (FMU) has also emerged. However, current FMU approaches often involve additional time-consuming steps and may not offer comprehensive unlearning capabilities, which renders them less practical in real FL scenarios. In this paper, we introduce FedAU, an innovative and efficient FMU framework aimed at overcoming these limitations. Specifically, FedAU incorporates a lightweight auxiliary unlearning module into the learning process and employs a straightforward linear operation to facilitate unlearning. This approach eliminates the requirement for extra time-consuming steps, rendering it well-suited for FL. Furthermore, FedAU exhibits remarkable versatility. It not only enables multiple clients to carry out unlearning tasks concurrently but also supports unlearning at various levels of granularity, including individual data samples, specific classes, and even at the client level. We conducted extensive experiments on MNIST, CIFAR10, and CIFAR100 datasets to evaluate the performance of FedAU. The results demonstrate that FedAU effectively achieves the desired unlearning effect while maintaining model accuracy. Our code is availiable at https://github.com/Liar-Mask/FedAU.

==> Section/Preliminary.tex <==



\section{Preliminary}
\subsection{Federated Learning}
% Federated learning was proposed by McMahan et al.~\cite{mcmahan2017communication}, aiming to build a machine learning model based on datasets that are distributed across multiple devices \cite{konevcny2016federated,mcmahan2017communication} without sharing private data with the server and other devices.  
Consider a Federated Learning \footnote{Federated learning refers to horizontal federated learning in this paper.} consisting of $K$ clients who collaboratively train a FL model $\omega$ to optimize the following objective:
\begin{equation} \label{eq:objective}
    \min_{\omega} \sum_{k=1}^K\sum_{i=1}^{n_k}\frac{\ell(F_\omega(x_{k,i}), y_{k,i})}{n_1+\cdots+n_K},
\end{equation}
where $\ell$ is the loss, e.g., the cross-entropy loss, $\calD_k=\{(x_{k,i}, y_{k,i})\}_{i=1}^{n_k}$ is the dataset with size $n_k$ owned by client $k$. 
%
In each communication round, client $k$ uploads their own model weights $\omega_k$ ($k=1,\cdots, K$) to the server and then the server aggregates all uploaded model weights through $\omega = \frac{1}{K}\sum_{k=1}^K\omega_k$. Next, the server distributes the aggregated weights to all clients 
(see the left of \Fref{fig:fm}).
% (see Fig. \ref{fig:Framework}(a)).

\subsection{Machine Unlearning}
Suppose a learning algorithm $A$ over $D$ outputs the model $A(D)$. An unlearning algorithm $\bar A$ takes
as input the model $A(D)$ and a set $D_u \subset D$ of data samples that are to be deleted, and is required to
output a new model $\Tilde{w}\in \calW$. We emphasize that the unlearning algorithm
does not have access to the entire original dataset $D$ in this resource-constrained setting and hence cannot retrain from scratch.
\begin{definition}{$(\epsilon, \delta)$-unlearning \cite{ginart2019making}.} For all $D$ of size $n$ and delete requests $D_u \subset D$ such that $|D_u| = m$, and $W \subset \calW$, a learning algorithm $A$ and an unlearning algorithm $\bar A$ is $(\epsilon, \delta)$-unlearning if
\begin{equation}
   Pr(A(D-D_u) \in W) \leq e^\epsilon Pr(\bar A(A, D_u, D) \in W) + \delta
\end{equation}
and 
\begin{equation}
    Pr(\bar A(A, D_u, D) \in W) \leq e^\epsilon Pr(A(D-D_u) \in W) + \delta
\end{equation}
    
\end{definition}
